Search for decays of neutral beauty mesons into four muons

A search for the non-resonant decays $B^0_s \rightarrow \mu^{+}\mu^{-}\mu^{+}\mu^{-}$ and $B^0 \rightarrow \mu^{+}\mu^{-}\mu^{+}\mu^{-}$ is presented. The measurement is performed using the full Run 1 data set collected in proton-proton collisions by the LHCb experiment at the LHC. The data correspond to integrated luminosities of $1$ and $2~\mathrm{fb}^{-1}$ collected at centre-of-mass energies of $7$ and $8~\mathrm{TeV}$, respectively. No signal is observed and upper limits on the branching fractions of the non-resonant decays at $95\%$ confidence level are determined to be \mathcal{B}(B^0_s \rightarrow \mu^{+}\mu^{-}\mu^{+}\mu^{-}) & < 2.5 \times 10^{-9} \mathcal{B}(B^0 \rightarrow \mu^{+}\mu^{-}\mu^{+}\mu^{-}) & < 6.9 \times 10^{-10}.

==> figures.tex <==
\section{Summary}
\label{sec:Summary}

